Latent Space Autoregression for Novelty Detection

Novelty detection is commonly referred to as the discrimination of observations that do not conform to a learned model of regularity. Despite its importance in different application settings, designing a novelty detector is utterly complex due to the unpredictable nature of novelties and its inaccessibility during the training procedure, factors which expose the unsupervised nature of the problem. In our proposal, we design a general framework where we equip a deep autoencoder with a parametric density estimator that learns the probability distribution underlying its latent representations through an autoregressive procedure. We show that a maximum likelihood objective, optimized in conjunction with the reconstruction of normal samples, effectively acts as a regularizer for the task at hand, by minimizing the differential entropy of the distribution spanned by latent vectors. In addition to providing a very general formulation, extensive experiments of our model on publicly available datasets deliver on-par or superior performances if compared to state-of-the-art methods in one-class and video anomaly detection settings. Differently from prior works, our proposal does not make any assumption about the nature of the novelties, making our work readily applicable to diverse contexts.

==> sections/legacy/experiments.tex <==
\begin{table*}[t]
\begin{center}
\begin{tabular}{|r|F|F|F|F|}
\hline
& MNIST & CIFAR10 & DR(eye)VE & ShanghaiTech\\\hline
E-blocks&[32,64]&[64,128,256]&[8,16,32,64,64]&[8,16,32,64,64]\\
D-blocks&[64,32]&[256,128,64]&[64,32,16,8,8]&[64,32,16,8,8]\\
Spatial stride&[2,2]&[2,2,2]&[2,2,2,2,2]&[2,2,2,2,2]\\
Temporal stride&-&-&[2,2,1,1,1]&[2,2,1,1,1]\\
FC-layers&[64]&[256,64]&[64]&[512,64]\\
MFC layers&[32,32,32,32,100]&[32,32,32,32,100]&-&-\\
MSC layers&-&-&[4,4,100]&[4,4,100]\\
Code dim&64&64&4$\times$64&4$\times$64\\
mini-batch&64&64&12&8\\\hline
\end{tabular}
\end{center}
\caption{Details regarding each implemented model. We report the number of encoder (E) and decoder (D) blocks along with the number of filter banks applied by each convolution, the stride of the first convolution within each encoder block (decoder mirrors the architecture, so strides are applied in reverse), the fully connected layers constructing the code, the number of channels of hidden autoregressive (MFC, MSC) layers,  the code dimensionality, the mini-batch size employed during training.}
\label{tab:model_details}
\end{table*}
%
\begin{table*}[t]
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|CCCCCC|C||CCCCCC|C|}
\hline
&\multicolumn{7}{c||}{MNIST}&\multicolumn{7}{c|}{CIFAR10}\\\cline{2-15}
& OC SVM & KDE & DAE & VAE & Pix CNN & GAN & AND & OC SVM & KDE & DAE & VAE & Pix CNN & GAN & AND\\\hline
0&0.988&0.885&0.991&0.998&0.531&0.926&0.993&0.630&0.658&0.411&0.700&0.788&0.708&0.717\\
1&0.999&0.996&0.999&0.999&0.995&0.995&0.999&0.440&0.520&0.478&0.386&0.428&0.458&0.494\\
2&0.902&0.710&0.891&0.956&0.476&0.805&0.959&0.649&0.657&0.616&0.679&0.617&0.664&0.662\\
3&0.950&0.693&0.935&0.950&0.517&0.818&0.966&0.487&0.497&0.562&0.535&0.574&0.510&0.527\\
4&0.955&0.844&0.921&0.966&0.739&0.823&0.956&0.735&0.727&0.728&0.748&0.511&0.722&0.736\\
5&0.968&0.776&0.937&0.959&0.542&0.803&0.964&0.500&0.496&0.513&0.523&0.571&0.505&0.504\\
6&0.978&0.861&0.981&0.995&0.592&0.890&0.994&0.725&0.758&0.688&0.687&0.422&0.707&0.726\\
7&0.965&0.884&0.964&0.978&0.789&0.898&0.980&0.533&0.564&0.497&0.493&0.454&0.471&0.560\\
8&0.853&0.669&0.841&0.907&0.340&0.817&0.953&0.649&0.680&0.487&0.696&0.715&0.713&0.680\\
9&0.955&0.825&0.960&0.982&0.662&0.887&0.981&0.508&0.540&0.378&0.386&0.426&0.458&0.566\\\hline
avg&0.951&0.814&0.942&0.969&0.618&0.866&0.975&0.586&0.610&0.536&0.583&0.551&0.592&0.617\\\hline
\end{tabular}}
\end{center}
\caption{ROC-AUC results for novelty detection on MNIST and CIFAR10. Each row represents a different class on which baselines and ANDs are trained on.}
\label{tab:oc_mnist_cifar}
\end{table*}
\section{Experiments}
\label{sec:experiments}
In this section we evaluate quantitatively the proposed AND model in two contexts: one class novelty detection and video anomaly detection. 
\\\\
{\bf Implementation details.} All experiments were performed following the general model illustrated in Sec.~\ref{sec:model}. However, some architectural choices were specialized for each dataset, in order to cope with different data complexities, overfitting or other issues. These modifications mainly involve the encoder and decoder capacities, in terms of convolutional blocks and number of filter banks within each block. We refer the reader to Tab.~\ref{tab:model_details} for more details. All models were trained minimizing Eq.~\ref{eq:loss} using $B=100$. As for the optimizer, we choose Adam~\cite{kingma2014adam}, with a learning rate of 0.001.
%
\subsection{Novelty detection: MNIST and CIFAR10}
%
\label{sec:oc_images}
We first assess the ability of our model to discriminate between normal samples seen during training and ones drawn from a different distribution. In these terms, we perform several one-class experiments on MNIST and CIFAR10. Specifically, for both datasets we isolate images from each class and consider them as the normal distribution. For each class, we train a different AND network and at test time, the whole test set is presented: the model is tasked to assign a higher score (probability) to samples sharing the class with training images. We randomly pick 20\% images from the training set of each class, and use it for validation purposes. Importantly, no novel samples are employed within the training and validation set. \\
%
\begin{figure*}[tb]
    \begin{center}
    \begin{tabular}{cc}
        Low density & High density \\
        \includegraphics[width=0.4\textwidth]{oneclass/cifar_ld} & \includegraphics[width=0.4\textwidth]{oneclass/cifar_hd}
    \end{tabular}
    \end{center}
    \caption{For each class in the CIFAR test set, we report images assigned to a low probability density (left image) and a high probability density (right image) by our model. High density images are clearly more regular than other ones, in terms of object size (airplanes, boats), context (deer) and orientation (horses).}
    \label{fig:cifar_regularity}
\end{figure*}
%
We consider the following baselines:
\begin{itemize}
    \item standard methods such as OC-SVM~\cite{scholkopf2000support} and Kernel Density Estimator (KDE), employed out of features extracted by PCA-whitening. Hyperparameters such as the number of principal components, the KDE kernel bandwidth and OC-SVM tolerance are tuned on the validation set.
    \item a denoising autoencoder (DAE), sharing the same encoder-decoder structure as our proposal, but defective of the density estimation module. The reconstruction error is employed as a measure of normalcy vs novelty.
    \item a variational autoencoder (VAE)~\cite{kingma2013auto}, also sharing the same capacity as our model, in which the Evidence Lower Bound (ELBO) is employed as score.
    \item an autoregressive model such as Pix-CNN~\cite{van2016conditional}, that estimates the density directly in the pixel space.
    \item the GAN-based approach illustrated in~\cite{schlegl2017unsupervised}.
\end{itemize}
Both baselines and our model feature unbounded scores, thus choosing a threshold to get a categorical prediction is often problematic. Therefore, Tab.~\ref{tab:oc_mnist_cifar} reports results of this experiment in terms of ROC-AUC. This metric can be interpreted as the expectation that a uniformly drawn normal image is scored higher than a uniformly drawn novel image, and is free from the choice of a fixed threshold.\\\\
%
Considering a simple setting such as MNIST, most methods perform favorably. 
In particular, VAE and AND yield the best results, and exhibit very similar performances. This is reasonable due to the fact that with such a clean image content the code distribution collapses to a simple distribution in the latent space for which the Naive Gaussian posterior imposed by VAE is a good proxy.
% Moreover, both the approaches share the similar autoencoding structure. 
% However, they differ in that VAE assumes a Gaussian prior over latent representations, while autoregression makes no assumption.
% Furthermore, VAE considers each element of the code to be independent from the others in terms of CPDs, whereas this is obviously differs from autoregression. 
Surprisingly, Pix-CNN excels in modeling the distribution of ones, but struggles on other classes. This finding suggests that autoregression within the joint space of pixels is complex, while employing it in representation space can be beneficial. Notably, OC-SVM outperforms most deep models in this setting.\\
%
On the contrary, CIFAR10 exhibits a strong intra-class variability and represents a significant challenge for most methods. Many baselines score lower or near 0.5 on many classes, which means similar or even worse than random scoring. In this setting, AND outperforms all baselines.
The gap with VAE increases, possibly due to the Gaussian posterior VAE assumes for latent representations, which represents a more severe constraint in the setting of real world images.
DAE performances suggest that reconstruction errors can indeed be interpreted as a proxy for sample density, but requires extra carefulness. Specifically, autoencoders are very likely to encode low-level features within the code (since they are useful for reconstruction), resulting in precise restorations of novel unseen samples. 
% On the contrary, AND models do not care about the level of abstraction of extracted representations, and directly model their distribution.
On the contrary, AND models directly model the density of extracted representations, regardless their level of abstraction, without making assumptions about their underlying distribution.
% The GAN approach in~\cite{schlegl2017unsupervised} scores favorably, especially when dealing with statistics from real-world images.
Notably, KDE yields a better performance with respect to all deep learning based approaches, except for AND. Nevertheless, KDE is a non-parametric estimator, therefore needs to store all training examples in memory in order to evaluate the normalcy of new images thus resulting an unfeasible approach as the dataset grows in size.\\
%
A visualization of AND behavior is represented in Fig.~\ref{fig:cifar_regularity}, illustrating CIFAR images scored with low and high densities.
%
\begin{table*}[t]
\begin{center}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|c|DDDDD|DDDDD|}
\hline
&\multicolumn{5}{c|}{ConvAE~\cite{hasan2016learning}}&\multicolumn{5}{c|}{AND}\\\cline{2-11}
& P@20 & P@50& P@100 & MAP & AUC & P@20 & P@50& P@100 & MAP & AUC\\\hline
Morning&0.85&0.72&0.58&0.513&0.713&0.95&0.88&0.87&0.570&0.758\\
Evening&0.50&0.68&0.65&0.466&0.700&0.00&0.00&0.00&0.366&0.662\\
Night&0.75&0.90&0.95&0.937&0.977&1.00&1.00&1.00&0.965&0.981\\
Sunny&0.60&0.50&0.44&0.368&0.529&0.95&0.48&0.40&0.409&0.585\\
Cloudy&0.60&0.62&0.59&0.470&0.583&0.85&0.80&0.71&0.507&0.626\\
Rainy&0.75&0.62&0.46&0.290&0.472&1.00&1.00&0.96&0.286&0.494\\
Downtown&0.15&0.14&0.21&0.344&0.414&0.15&0.20&0.19&0.336&0.441\\
Countryside&0.30&0.42&0.34&0.326&0.506&1.00&1.00&0.98&0.561&0.721\\
Highway&0.60&0.36&0.48&0.367&0.632&1.00&1.00&1.00&0.525&0.718\\\hline
avg&0.57&0.56&0.52&0.453&0.614&\textbf{0.77}&\textbf{0.71}&\textbf{0.68}&\textbf{0.473}&\textbf{0.665}\\\hline
\end{tabular}}
\end{center}
\caption{Performances on the DR(eye)VE novelty detection task.}
\label{tab:oc_dreyeve}
\end{table*}
%
\begin{figure*}[bth]
\begin{center}
\begin{tabular}{c@{\hskip 0.15in}c@{\hskip 0.15in}c}
\includegraphics[width=0.25\textwidth]{images/dreyeve_aucs/tod}&
\includegraphics[width=0.25\textwidth]{images/dreyeve_aucs/weather}&
\includegraphics[width=0.25\textwidth]{images/dreyeve_aucs/landscape}
\end{tabular}
\end{center}
\caption{ROC curves representing AND and ConvAE~\cite{hasan2016learning} performances on the DR(eye)VE dataset, aggregated by time of day, weather and landscape.}
\label{fig:dreyeve_aucs}
\end{figure*}
%
\begin{figure*}[tb]
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{EEEEEEEEE}
\hline
\multicolumn{9}{c}{High scored clips for the normal class}\\\hline
Morning&Evening&Night&Sunny&Cloudy&Rainy&Downtown&Countryside&Highway\\
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_0_corrects}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_1_corrects}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_2_corrects}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_3_corrects}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_4_corrects}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_5_corrects}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_6_corrects}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_7_corrects}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_8_corrects}\\\hline\hline
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_0_mistakens}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_1_mistakens}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_2_mistakens}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_3_mistakens}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_4_mistakens}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_5_mistakens}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_6_mistakens}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_7_mistakens}&
\includegraphics[width=0.17\textwidth]{images/oneclass/dreyeve/class_8_mistakens}\\
(Evening)&(Night)&(Evening)&(Rainy)&(Rainy)&(Cloudy)&(Highway)&(Highway)&(Countryside)\\\hline
\multicolumn{9}{c}{High scored clips for a novel class}\\\hline
\end{tabular}}
\end{center}
\caption{Analysis of AND errors in the DR(eye)VE novelty detection task. Each column illustrates high scored clips of a model trained on a single scenario. The topmost image of each column reports the first frame of the normal clip yielding the highest score. The bottom image reports the first frame of the clip yielding the highest scores among the novel classes. Best viewed on screen and zoomed in.}
\label{fig:dreyeve_errors}
\end{figure*}
%
\subsection{Novelty detection: DR(eye)VE}
%
We now stress AND performances in a more challenging video novelty detection context. We employ the recently proposed DR(eye)VE dataset~\cite{dreyeve2016} which features 74 sequences of driving videos, from the perspective of a car, each of which is 5 minutes long. The dataset was originally proposed for attention prediction but releases, for each sequence, annotations concerning the type of landscape (downtown, countryside, highway), the time of acquisition (morning, evening, night) and weather (sunny, cloudy, rainy). Therefore, we proceed in a similar fashion as presented in Sec.~\ref{sec:oc_images}, training several AND models by isolating each class and successively assessing their ability to recognize normal and novel samples. The network is fed with 16-frames clips, with images down-sampled to match a resolution of $160\times256$ pixels. For training, we employ clips randomly drawn from the first 38 driving sequences (except for the central 500 frames), while the test set is composed of 10000 random clips from the remaining ones. 200 random clips from the 500 central frames of each training sequence constitute the validation set. We report in Tab.~\ref{tab:oc_dreyeve}, Fig.~\ref{fig:dreyeve_aucs} AND results compared to the convolutional autoencoder (ConvAE) approach presented in~\cite{hasan2016learning}, which scored favorably in several video benchmarks. Evaluation is carried out by sorting test samples according to the predicted normalcy score, and computing precision@k (P@K), mean average precision (MAP) and ROC-AUC. As shown in table, AND outperforms the competitor model on nearly all classes. In particular, it clearly emerges how \quotes{night} clips are easy to distinguish from \quotes{morning} and \quotes{evening} ones, due to global changes in illumination. On the other hand, classes such as \quotes{rainy} and \quotes{downtown} yield poor performances. 

%
In particular, two degenerate cases needs further reasoning. Indeed, \quotes{evening} sequences score positively globally, but have zero precision in the first 100 test samples. This is again due to global illumination, in that AND tends to positively score darker images, which correspond to \quotes{night} within the test set. The opposite case is represented by \quotes{rainy} sequences, where scores are not discriminative globally but very precise in terms of top precisions. This suggests highly distinctive clips within rainy sequences (e.g. where the camera itself is covered by water drops), in spite of many others that are very hard to distinguish i.e. when light rain falls and drops are not visible in the clip.
To represent the task complexity and a qualitative analysis of AND errors, we report in Fig.~\ref{fig:dreyeve_errors} the best-scoring normal clip and the best-scoring novel clip for each class. The figure illustrates, column-wise, that the boundary separating a class from other ones is often mild. As an example, \quotes{night} can be easily mistaken for \quotes{evening} when the illumination condition is similar, and discriminating between \quotes{cloudy} and \quotes{rainy} is generally hard. 
%
\begin{figure*}[tb]
\begin{center}
\begin{tabular}{lr}
\includegraphics[width=0.45\textwidth]{images/stech/st_01_0051}&
\includegraphics[width=0.45\textwidth]{images/stech/st_06_0144}\\
\includegraphics[width=0.45\textwidth]{images/stech/st_07_0049}&
\includegraphics[width=0.45\textwidth]{images/stech/st_12_0174}\\
\end{tabular}
\end{center}
\caption{Representation of AND behavior on four sequences of the Shanghai Tech test set. We plot the negative log-probability (NLP) predicted by our model for each frame. It can be considered a measure of anomaly (the highest, the more abnormal) and succeeds in detecting different unusual behaviors. Best viewed on screen and zoomed in.}
\label{fig:ad_stech}
\end{figure*}
\subsection{Video anomaly detection}
A further domain interested by the proposed autoregressive model is video anomaly detection. This topic has a great impact on many computer vision applications, including surveillance, where it is often cast as the detection of uncommon pedestrian's moving patterns. We are interested in evaluating whether our density estimation approach transfers to this peculiar setting where the anomaly is triggered by the temporal evolution of small scene regions (i.e. where pedestrians behave).\\
%
For the purpose, we choose the recent Shanghai Tech Campus benchmark~\cite{luo2017revisit}. The dataset features 13 different cameras, delivering more than 250,000 frames for training, and 130 clips representing abnormal events for testing. These latter ones comprehend appearances of bicicles, cars and other vehicles, as well as hasty changes in motion patterns due to episodes of chasing, brawling, fighting, and pick pocketing.\\
During test, we evaluate 16-frames clips seeking for a frame level score. Thus, we compute the score of a frame as the mean score among the 16 clips containing it.
\begin{table}[b]
\begin{center}
\begin{tabular}{|r|c|}
\hline
& ROC-AUC\\\hline
ConvAE~\cite{hasan2016learning}& 0.609 \\
TSC~\cite{luo2017revisit}& 0.679 \\
sRNN~\cite{luo2017revisit} & 0.680 \\\hline
AND & \textbf{0.685}\\\hline
\end{tabular}
\end{center}
\caption{Results on Shanghai Tech Campus anomaly detection benchmark, where AND performs on par with other state of the art models.}
\label{tab:stech}
\end{table}
We report our performances in Tab.~\ref{tab:stech}, compared to ConvAE model by Hasan~\etal~\cite{hasan2016learning},  Temporally-coherent Sparse Coding (TSC) and stacked RNN (sRNN) from~\cite{luo2017revisit}. During testing, we notice how sequences from different cameras were scored differently due to the distribution of training clips. Coherently with its objective, our model tends to assign a higher score to cameras delivering more sequences. Nevertheless, within a given sequence abnormal behaviors are generally detected. We compute the ROC-AUC separately for each sequence and report the mean. Notably, our model outperforms ConvAE by a significant margin, and performs on par with other state-of-the-art models. This result is remarkable for two reasons: the first is that we do not make any assumption about surveillance specific features set (e.g. optical flow like in~\cite{xu2017detecting}), but instead the autoencoder seamlessly focuses on motion features; eventually anomalies emerge directly from the modeling of latent distributions without any assumption about both their structure and domain.\\
%
We report in Fig.~\ref{fig:ad_stech} some success cases, in which AND successfully identifies abnormal entities such as bycicles and cars, as well as uncommon behaviors such as brawling.
%
\begin{table*}[tbh]
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|DDDDDDDDDD|}
\hline
\multicolumn{2}{|c|}{}&\multicolumn{10}{c|}{Classes}\\\cline{3-12}
\multicolumn{2}{|c|}{}&0&1&2&3&4&5&6&7&8&9\\\hline
\multirow{3}{*}{ARG}&Train&-201.60&-161.60&-171.43&-172.73&-174.17&-186.48&-158.22&-162.37&-171.65&-154.11\\
&Val&-200.96&-160.38&-170.10&-172.29&-173.85&-185.25&-157.22&-162.20&-171.42&-154.02\\
&Test&-200.89&-159.73&-169.64&-170.75&-172.40&-184.27&-157.74&-161.65&-170.10&-152.70\\\hline
\multirow{3}{*}{RDM}&Train&-496.33&-456.34&-466.16&-467.47&-468.90&-481.21&-452.95&-457.10&-466.39&-448.84\\
&Val&-495.69&-455.11&-464.83&-467.02&-468.58&-479.98&-451.95&-456.93&-466.15&-448.75\\
&Test&-495.62&-454.47&-464.37&-465.48&-467.13&-479.00&-452.48&-456.38&-464.83&-447.43\\\hline
\multirow{3}{*}{INV}&Train&-791.06&-751.07&-760.89&-762.20&-763.63&-775.94&-747.68&-751.83&-761.12&-743.57\\
&Val&-790.42&-749.84&-759.56&-761.75&-763.31&-774.71&-746.68&-751.66&-760.88&-743.48\\
&Test&-790.35&-749.20&-759.11&-760.22&-761.86&-773.73&-747.21&-751.12&-759.56&-742.16\\\hline
\end{tabular}}
\end{center}
\caption{Average log-likelihood numerical results. Each BN is trained on AND latent codes from the training set of a single class, following either the autoregression order (ARG), a random order (RDM) or the order inverse to autoregression (INV). We report the log-likelihood also on the validation and test set. For train-val-test split, see Sec~\ref{sec:oc_images} of the paper. Only \quotes{normal} test samples are used in this evaluation.}
\label{tab:bn_log_likelihood}
\end{table*}
%
\subsection{On the causal structure of representations}
%
In this section we investigate the capability of the AND encoder to produce representations that follow the causal structure imposed by the autoregression loss during training. To this aim, we extract representations out of the 10 AND models trained on MNIST digits (Sec.~\ref{sec:oc_images}) and fit different graphical models to model their distribution. Specifically, we train several Bayesian Networks (BNs), with different autoregressive structures. Specifically, each BN is modeled with Linear Gaussian CPDs~\cite{koller2009probabilistic}, such that the CPD $P(Y/Pa(Y))$ is modeled as
\begin{equation}
Y \sim \mathcal{N}(w_o + \sum_{X_i \in Pa(Y)} w_iX_i;\sigma^2)
\end{equation}
with the exception of root nodes that are modeled with a Gaussian distribution. 
%
Concerning the ordering, we test:
\begin{itemize}
    \item \textbf{ARG} order: the BN structure follows the autoregressive order imposed during training.
    \item \textbf{RDM} order: the BN structure follows a random autoregressive order.
    \item \textbf{INV} order: the BN structure follows an autoregressive order which is the inverse with respect to the one imposed during training.
\end{itemize}
It is worth noticing that the three structures exhibit the same number of edges and independent parameters, so that the difference in fitting capabilities is only due to the causal order imposed over variables.\\
%
Fig.~\ref{fig:bn_likelihood} reports the average training log-likelihood (i.e. the training log-likelihood divided by the number of training samples) of all BN models. Remarkably, the autoregressive order is clearly a better fit, supporting the capability of the encoder network to extract features with known autoregressive properties. Moreover, to show that this result is not due to overfitting or other lurking behaviors, we report in Tab~\ref{tab:bn_log_likelihood} log-likelihoods for training, validation and test set (as defined in Sec.~\ref{sec:oc_images}).
%
\begin{figure}[b]
\begin{center}
\includegraphics[width=0.8\columnwidth]{images/bn/nll_MNIST}
\end{center}    
\caption{Average training log-likelihood of a Bayesian Network modeling the distribution of latent codes produced by the AND encoder (trained on MNIST digits). When the network structure resembles the autoregressive order imposed during AND training, a much higher likelihood is achieved. This behavior is consistent in all classes, and supports the capability of the AND encoder to produce codes that respect a pre-imposed autoregressive structure.}
\label{fig:bn_likelihood}
\end{figure}
%



==> sections/legacy/introduction.tex <==
\section{Introduction}
%The definition of novelty has challenged the humankind since pre-platonian theories of knowledge \cite{plato paradoxes of meno}.    
Novelty and anomaly detection have been extensively studied in computer vision since many years. Nonetheless, the cornerstone of research in the field is the definition of novelty itself. The concept of discovering novelty has emerged since Greek philosophy in the popular Plato's paradox of inquiry, where the philosopher raised the question \quotes{how can I know something that I didn't know before?}. Hence, the problem of novelty can be apprehended as the problem of knowledge~\cite{brioschi2015problem}. 
Accordingly, novelty detection in computer science was defined as \quotes{the identification of \emph{unknown} data or signals that a machine learning system is not \emph{aware} of during training}~\cite{MARKOU20032499,AHMED201619}. 
%Though, it is directly linked with the lack of knowledge falling into the Plato's paradox. 
% Similarly, anomaly detection in computer vision has been mostly associated with the concept of events or actions that are different with respect to \emph{known} models, assuming that the anomaly is given by an object, a person or a group of targets which behave in a \emph{surprising} manner~\cite{Chandola}.\\
In computer vision this has been mostly associated with events or actions that are different with respect to \emph{known} models, e.g. referring to an object, a person or a group of targets which behave in a \emph{surprising} manner~\cite{Chandola}.\\
In this work we tackle this problem by modelling the knowledge by means of a probability distribution for which \quotes{novel} elements are the most inexplicable ones in a probabilistic sense. This formulation abides both conventional computer science definition and classical novelty interpretations.
Technically, this is achievable through an unsupervised knowledge distiller that summarizes the actual informative content about the data and simultaneously models its probability distribution. 
To this aim, we leverage the power of deep autoencoders as effective knowledge compressors, while forcing autoregressive properties on distilled codes in order to estimate their density function.
Despite autoregressive density estimation have been profitably applied to deep learning~\cite{larochelle2011neural,uria2013rnade,germain2015made}, our contribution resides in an holistic approach where the extracted knowledge is conditioned to follow an autoregressive scheme thus its probability can be captured during training.
We evaluate our Autoregressive Novelty Detector (AND) on both image and video novelty and anomaly detection tasks achieving very encouraging results.
To the best of our knowledge, this is the first model employing autoregression for the estimation of density functions in complex, high dimensional feature spaces. We believe the proposed procedure can foster many possible refinements in several different applications processing highly structured and dimensional data.

==> sections/legacy/model.tex <==
\section{Proposed model}
\label{sec:model}
\begin{figure}[tb]
\begin{center}
\resizebox{0.8\columnwidth}{!}{%
\begin{tikzpicture}[
    ->,
    >=stealth',
    auto,node distance=0.15\textwidth,
    thick,
    main node/.style={circle, draw, font=\sffamily\large\bfseries, inner sep=1}
    ]
 \node[main node] (1) {$X_1$};
  \node[main node] (2) [right of=1] {$X_2$};
  \node[main node] (3) [right of=2] {$X_3$};
  \node[main node] (4) [right of=3] {$X_4$};

  \path[every node/.style={font=\sffamily\small}]
    (1) edge node [right] {} (2)
    (2) edge node [right] {} (3)
    (3) edge node [right] {} (4);
  \draw (1) [out=30,  in=150] to (3);
  \draw (1) [out=30,  in=150] to (4);
  \draw (2) [out=330,  in=210] to (4);
\end{tikzpicture}}
\end{center}
\caption{An example of autoregression over the joint probability distribution of four variables, represented as a graphical model. According to this model, estimating the joint probability of $X_1$, $X_2$, $X_3$, $X_4$ reduces to the estimation of the conditionals $P(X_4|X_3X_2X_1)$, $P(X_3|X_2X_1)$, $P(X_2|X_1)$ and the marginal $P(X_1)$.}
\label{fig:autoregression}
\end{figure}
%
In this section we describe the proposed model, according to which the scoring function is a probability density estimator, that directly learns to assign high probabilities to normal samples within the training set. The learned density function evaluates representations produced by a deep autoencoder, and its estimation proceeds following an autoregressive procedure, in which elements of the feature vector get observed gradually to predict the value of unobserved ones. 
First, we briefly review the technique of autoregression and its application in density estimation. Afterwards, the model's architecture and objective function will be illustrated in detail.
%
\begin{figure*}[tb]
\begin{center}
\includegraphics[width=0.7\textwidth]{model/model}
\end{center}
\caption{The structure of the proposed autoencoder. Paired with a standard compression-reconstruction network, a density estimation module learns the distribution of latent codes, via autoregression.}
\label{fig:model}
\end{figure*}
%
\subsection{Background: autoregressive models}
Autoregression is a well known technique that factorizes the probability distribution over the joint assignment $\textbf{x}$ of $D$ random variables using the chain rule of probability,
\begin{equation}
\label{eq:autoregression}
p(\textbf{x})= \prod_{d=1}^D p(x_d|\textbf{x}_{<d}),
\end{equation}
%
so that estimating $p(\textbf{x})$ reduces to the estimation of each single conditional probability density (CPD) in the form $p(x_d|\textbf{x}_{<d})$. Notably, Eq.~\eqref{eq:autoregression} assumes a given order over random variables (Fig.~\ref{fig:autoregression}). Despite the chain rule is true in general, estimating CPDs can be easier for some peculiar variable ordering and harder for others, depending on the nature of the joint variable space. Prior models such as Pixel-RNN~\cite{oord2016pixel} and Pixel-CNN~\cite{van2016conditional} employ autoregression to generate images one pixel at a time, and the ordering in which the process advances is either from corners to center or top-left to bottom-right, row-wise. 
% This is reasonable due to the structure of natural images, that are mostly composed of compact objects. 
Other autoregressive models \cite{uria2014deep,germain2015made} perform order agnostic training by shuffling the order at each mini-batch update. A lot of efforts have been spent in this direction, because all mentioned models estimate the density of raw data, for which the best autoregressive order is unknown. On the contrary, we employ this technique out of representations extracted by a deep network, that we constrain to provide autoregressive feature vectors.
%
\subsection{Autoregressive novelty detection}
The successful application of autoregression in density estimation motivates us in employing it in a novelty detection setting. However, in real world scenarios this requires modeling of extremely high dimensional data (e.g. images and videos). This can be troublesome for two reasons: First, as the dimensionality of the feature space grows, the estimation of a density function gets more and more difficult as the number of required samples raises significantly. Moreover, since each autoregressive layer requires at least the same number of hidden units as the input layer~\cite{germain2015made}, the scalability of the whole model turns unfeasible due to memory limitations and the exploding number of parameters.\\
%
We deal with the aforementioned problems by shifting the analysis in a compressed domain i.e. the feature space learned by a deep autoencoder. This way, data dimensionality problems are alleviated, since autoencoders can significantly compress input data. More importantly, by forcing the autoregression property during the autoencoder training, it is possible to guide the feature space creation, such that the encoded representation is autoregressive in any preset order.
%
More formally, our architecture is composed of three building blocks (Fig.~\ref{fig:model}): the encoder $f({\bf x};{\bf \theta}_f)$, the decoder $g({\bf z};{\bf \theta}_g)$ and the density estimator $h({\bf z};{\bf \theta}_h)$. The encoder processes input ${\bf x}$ from an unknown training distribution $p(x)$ and maps it into a compressed representation ${\bf z} = f({\bf x};{\bf \theta}_f)$, having lower dimensionality $D$, whereas the decoder provides a reconstructed version of the input $\tilde{{\bf x}} = g({\bf z};{\bf \theta}_g)$. Importantly, the representation ${\bf z}$ is sigmoid-activated, so that ${\bf z}\in [0,1]^D$. The estimator $h({\bf z};{\bf \theta}_h)$ provides the representation space density in ${\bf z}$ with autoregression. Specifically, it produces as output $D$ probability distributions $p(z_j)$, represented as multinomials over a linear quantization of the space $[0,1]$ in $B$ bins. In order to represent a proper probability distribution, a softmax activation is employed, ensuring that probabilities sum up to 1 along the quantization axis. As will be further detailed in the remainder of this section, all layers of the estimation network follow a precise connectivity scheme, ensuring that each output distribution $p(z_j)$ is only connected to inputs $\{z_1, \ldots, z_{j-1}\}$, thus resembling a valid autoregressive estimate of the CPD $p(z_j|{\bf z}_{<j})$.\\
%
\begin{figure*}[tb]
\begin{center}
\includegraphics[width=1\textwidth]{model/blocks}
\end{center}
\caption{Each block within the encoder and decoder network is composed of a convolutional path and an identity path, merged by a residual connection. For each convolutional layer, $s$ indicates the stride and $k$ the kernel size.}
\label{fig:blocks}
\end{figure*}
%
The objective of the complete architecture is to minimize:
%trained to minimize 
% \begin{align}
% \begin{split}
% \label{eq:loss}
%     L(\theta_f, \theta_g, \theta_h) = &\underbrace{\sum_{i=1}^N||{\bf x}^{(i)} - \tilde{{\bf x}}^{(i)}||^2}_\text{reconstruction loss} + \\
%     &\underbrace{\sum_{i=1}^N\sum_{j=1}^D\sum_{k=1}^B \phi({\bf z}_j^{(i)})_k \log(p({\bf z}_j^{(i)})_k)}_\text{autoregression loss},
% \end{split}
% \end{align}
\begin{align}
\begin{split}
\label{eq:loss}
    L(\theta_f, \theta_g, \theta_h) = \mathbb{E}_{p(x)}\bigg[&\underbrace{||{\bf x} - \tilde{{\bf x}}||^2}_\text{reconstruction loss} + \\
    &\underbrace{\sum_{j=1}^D\sum_{k=1}^B \phi({\bf z}_j)_k \log(p({\bf z}_j)_k)}_\text{autoregression loss}\bigg],
\end{split}
\end{align}
where $i$ spans over all $N$ training examples and $\phi(\cdot)$ is a utility function transforming each element $z_j$ into a $B$-dimensional one-hot encoding, highlighting the correct quantization bin to which $z_j$ belongs. Importantly, while the reconstruction loss guides the autoencoder $g(f({\bf x}; \theta_f);\theta_g)$ towards data compression, the autoregression loss trains the sub-network $h(f({\bf x}; \theta_f);\theta_h)$ to regress the distribution of compressed representations, through maximum likelihood estimation. Thus, the encoder's parametrization $\theta_f$ is forced to encode input samples such that representations are both descriptive (reconstruction loss is low) and lie in a high density region of the feature space (autoregression loss is low). Similar to the case of variational autoencoders~\cite{kingma2013auto}, the autoregression loss acts as a regularizer, avoiding the needs of other regularization techniques such as denoising and contraction.\\
%
\begin{figure*}
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc}
\includegraphics[width=0.45\textwidth]{images/model/mfc}&
\includegraphics[width=0.62\textwidth]{images/model/mconv}\\
(a)&(b)
\end{tabular}}
\end{center}
\caption{(a) Representation of a masked fully connected layer, described by Eq.~\ref{eq:mfc}. The connectivity between the input and output tensor is highlighted by different colors. We illustrate a layer of type A in this figure. (b) The Masked Stacked Convolutional layer (Eq.~\ref{eq:conv_stack}). It allows to exploit translation invariance only along the time axis. Different kernel colors represent different parametrizations.}
\label{fig:custom_layers}
\end{figure*}
%
Once the model is trained, we detach the decoder and interpret $h(f({\bf x}; \theta_f);\theta_h)$ as a deep density estimator, that can be queried with new samples for their plausibility under the learned distribution.
Indeed, the autoregression loss of a single test sample estimates the negative log-probability of its representation in feature space, hence can be used as a score for novelty versus regularity.\\\\
{\bf General architecture.}
The proposed model is represented in Fig.~\ref{fig:model}. The encoder and decoder networks are composed of several residual convolutional blocks, whose routing patterns require two paths. The standard path processes input by three stacked convolutions, the first of which changes the resolution of the input tensor (spatially and/or temporally) by striding, either down-sampling (encoder block) or up-sampling (decoder block, in which the first convolution of the block is transposed) feature maps. 
% Each convolution is followed by a batch normalization~\cite{ioffe2015batch} and a leaky ReLU activation, except for the last one that is linearly activated. 
An identity path proceeds by applying a strided unary kernel convolution. 
% The purpose of latter path is to resemble as closely as possible an identity, in order to improve the backward propagation of gradients towards previous blocks~\cite{he2016deep}.
Two densely connected sub-networks map the encoder output to the compressed feature vector and bring it back to a spatial feature map fed as input to the decoder. Further details about blocks are given in Fig.~\ref{fig:blocks}. 
\\\\
{\bf Image model.}
%
The network estimating image densities is composed of 2D blocks (Fig.~\ref{fig:blocks}, image model), except for the innermost layers that are fully connected and provide a compressed representation.
This compressed feature vector has dimensionality $D$ and, as mentioned, undergoes an autoregressive module that estimates its probability. Each layer within this module features a Masked Fully Connection (MFC, Fig.~\ref{fig:custom_layers}a), that can follow two different patterns, namely A and B. 
Formally, it computes output feature map ${\bf o} \in \mathbb{R}^{D\times co}$ given the input ${\bf h} \in \mathbb{R}^{D\times ci}$. The connection between the input element ${\bf h}_i^k$ in position $i$, channel $k$ and the output element ${\bf o}_j^l$ in position $j$, channel $l$ is parametrized by 
\begin{align}
\label{eq:mfc}
    \begin{cases}
    w_{i, j}^{k, l} &\quad \text{if $i < j$, type = A}\\
    0 &\quad \text{if $i \geq j$, type = A}\\
    w_{i, j}^{k, l} &\quad \text{if $i \leq j$, type = B}\\
    0 &\quad \text{if $i > j$, type = B}
    \end{cases}
\end{align}
The feature vector entering the first autoregressive layer hasn't any feature channel axis, thus it can be thought as a vector in $\mathbb{R}^{D \times 1}$. On the contrary, the output of the final autoregressive layer provides probability estimates for the $B$ bins that compose the space quantization (see previous section), so it lives in $\mathbb{R}^{D \times B}$. Intermediate layers can have an arbitrary number of output channels. The first layer within the estimation network has type A (thus strictly depending on previous elements), whereas all the remaining ones have type B (thus masking only successive elements). All hidden layers are leaky ReLU activated.
\\\\
{\bf Video model.}
When processing video inputs, the network consumes temporal clips of 16 consecutive frames. 
All convolutions are 3D, so they stride along the temporal axis~\cite{tran2015learning}. The structure of 3D blocks is represented in Fig.~\ref{fig:blocks}, video model. 
In order to obtain a temporally-ordered representation of the input clip, each 3D convolution within encoding blocks is \emph{causal}~\cite{BaiTCN2018}, so that the output cannot access information from future frames (i.e. each connection to future units is zero-masked).
The last fully connected layers within the encoder process each feature map along the temporal axis in parallel, so that maps from different time-steps undergo the same parametrization. This way, the encoding procedure does not shuffle information across time-steps, ensuring temporal ordering. The decoder architecture mirrors the encoder to restore the input data.\\
%
% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.65\textwidth]{images/model/mconv}
%     \caption{The Masked Stacked Convolutional layer (Eq.~\ref{eq:conv_stack}). It allows to exploit translation invariance only along the time axis. Different kernel colors represent different parametrizations}
%     \label{fig:msc}
% \end{figure}
The compressed representation of video clips has dimensionality $D=t\times d$, being $t$ the number of temporal time-steps and $d$ the length of the code. Accordingly, the estimation network is designed to capture two dimensional patterns within observed elements of the code in order to provide an estimate over the values of unobserved ones. 
% Therefore, each layer within it, is composed of masked 2D convolutions. 
However, naively plugging 2D convolutional layers would assume translation invariance in patterns that characterize the code.
Due to the way the compressed representation is built, this assumption is true only along the temporal axis, whereas it seems wrong along the code axis (as mentioned above, it is the output of a fully connected layer). To address these constraints, our proposal is to apply $d$ different convolutional kernels to each element along the code dimension, allowing the observation of the whole feature vector in the previous time-step and a portion of the current time-step (Fig.~\ref{fig:custom_layers}b). Every convolution is free to stride along the time axis, and captures temporal patterns. We name this operation Masked Stacked Convolution.\\
%
Specifically, the $i$-th convolution is equipped with a kernel ${\bf w}^{(i)} \in \mathbb{R}^{3\times d}$ kernel, that gets multiplied by the binary mask ${\bf M}^{(i)}$, defined as 
\begin{equation}
\label{eq:conv_mask}
m_{j,k}^{(i)}\in {\bf M}^{(i)}=
\begin{cases}
1 \quad \text{if $j=0$}\\
1 \quad \text{if $j=1$ and $k<i$ and type=A}\\
1 \quad \text{if $j=1$ and $k\leq i$ and type=B}\\
0 \quad \text{otherwise,}
\end{cases}
\end{equation}
where $j$ indexes the temporal axis and $k$ the code axis.\\
%
Each single convolution yields a column vector, as a result of its stride along time. The set of column vectors resulting from the application of the $d$ convolutions to the input tensor ${\bf h} \in \mathbb{R}^{t\times d \times ci}$ are horizontally stacked to build the output tensor ${\bf o} \in \mathbb{R}^{t\times d \times co}$, as follows:
\begin{equation}
\label{eq:conv_stack}
{\bf o}=\concat\limits_{i=1}^{d} [({\bf M}^{(i)}\odot {\bf w}^{(i)})\ast {\bf h}],
\end{equation}
where $||$ represents the horizontal concatenation operation.\\
%
Similarly to the model discussed for images, each MSC layer features a leaky ReLU activation and provides for one among two types of masking, namely A and B, the former employed only in the first layer and the latter employed in all successive layers within the estimation network. The output of the estimation network is a tensor having shape $t\times d\times B$ providing autoregressive CPDs for each element of the $t\times d$ representation of the input video clip.

==> sections/legacy/related.tex <==
\section{Related work}
\label{sec:related}
{\bf Novelty and anomaly detection in vision.}
Due to the complexity in defining and labeling novel events, nearly all methods in literature are based on unsupervised learning. Few models detect unusual patterns in data streams by employing statistical tests paired with either compressed sensing~\cite{budhaditya2009effective} or dimensionality reduction~\cite{pham2011detection}.
A significant line of work focuses on learning a parametric compression and reconstruction of normal data, motivated by the assumption that outlier samples lead to worse reconstructions. Among these approaches, sparse-coding algorithms model normal patterns as a linear combination of a set of basis components, imposing a sparsity constraint on scalar coefficients~\cite{zhao2011online,cong2011sparse,lu2013abnormal,xiao2015learning}.
On a different note, other models rely on learning the probability distribution of normal patterns by proposing both non-parametric~\cite{adam2008robust} and parametric~\cite{basharat2008learning,mahadevan2010anomaly,li2014anomaly} estimators to approximate the density of low-level appearance and motion features.
At a higher abstraction level, graphical modeling has proven successful in estimating the distribution of video events and their causality, by means of Hidden Markov Models~\cite{duong2005activity}, Markov Random Fields~\cite{kim2009observe} and energy-based models~\cite{kwon2015unified}.
% Other works like the social force model~\cite{mehran2009abnormal} or spectral graph analysis~\cite{calderara2011detecting} specifically address video surveillance scenarios, by tackling the detection of abnormalities in crowd trajectories patterns.
Other models, such as social force~\cite{mehran2009abnormal} and spectral graph analysis~\cite{calderara2011detecting}, specifically address video surveillance scenarios by tackling the detection of abnormalities in crowd trajectories patterns.
Finally, different directions involve clustering of spatio temporal video volumes~\cite{zhong2004detecting,roshtkhari2013online}, Gaussian Process Regression~\cite{cheng2015video}, scan statistics~\cite{hu2013unsupervised}, foreground explainability~\cite{antic2011video} and discriminability of normal frames with respect to context~\cite{del2016discriminative}.\\
Nevertheless, all aforementioned methods are disentangled by the feature extraction process and strongly depend on the efficacy of the chosen features set.
%
Modern novelty detection leverages the representation power of deep neural networks in the expense of hand crafted features. 
Algorithms such as one-class support vector machines (OC-SVM)~\cite{scholkopf2000support} or Gaussians classifiers have been successfully employed out of features extracted by deep networks~\cite{seebock2016identifying,xu2017detecting,sabokrou2015real,SABOKROU2018}.
Reconstruction-based models, instead, that  include autoencoders~\cite{hasan2016learning}, convolutional long-short term memories~\cite{medel2016anomaly} and sparse coding with temporal constraints~\cite{luo2017revisit}, have been employed by leveraging on the magnitude of the reconstruction error. Nevertheless, this metric has proven to be a proxy of the gradient of the log-density of hidden representations, rather than representing the density itself~\cite{alain2014regularized}.
%Gaussian classifiers have been employed out of features extracted either by autoencoders~\cite{sabokrou2015real} or deep convolutional neural networks pre-trained for classification~\cite{sabokrou2016fully}.
Few works address novelty detection by assessing temporal regularity of deep representations, by slow feature analysis~\cite{hu2016video} or binary temporal patterns~\cite{ravanbakhsh2016plug}.
Probabilistic models typically aim at estimating densities in deep feature space by means of GMMs~\cite{feng2017learning,zong2018deep}, or minimizing energy functions~\cite{zhai2016deep,vu2017energy}.
Indeed, GMMs expectation-maximization in high dimensions is troublesome, mostly due to the estimation of covariance matrices~\cite{zhu2017high,wang2015high,krishnamurthy2011high}.
Notably, the method in~\cite{nam2015direct} illustrates how CNNs can directly estimate density ratios of normalcy over novelty.
Motivated by their effectiveness in learning complex distributions, some recent works train generative adversarial networks (GANs) on normal samples. However, since the underlying data probability distribution is embedded in the network parameters and cannot be explicitly queried for scoring samples, these methods employ different heuristics for the evaluation. Specifically,~\cite{schlegl2017unsupervised,ravanbakhsh2017abnormal} employ reconstruction measures to monitor abnormalities, whereas~\cite{ravanbakhsh2017training} directly queries the GAN discriminator for a normalcy score.  
Finally, \cite{perera2018learning} addresses a related task, namely one-class classification, by learning CNN features that are both compact and descriptive using supervision from an additional external dataset.
\\
For a comprehensive review of anomaly detection techniques in computer vision, we refer the reader to~\cite{popoola2012video,kiran2018overview}.\\\\
%
{\bf Autoregressive density estimation}
A popular deep model for density estimation is the Restricted Boltzmann
Machine~\cite{smolensky1986information,freund1992fast}, which can be trained with contrastive divergence~\cite{hinton2002training} to model the density of binary inputs. The problem with this approach is that exact inference is troublesome due to an intractable partition function. To overcome this limitation, the first autoregressive models were introduced: the binary NADE~\cite{larochelle2011neural} and its real-valued version RNADE~\cite{uria2013rnade} employ a deep network to estimate conditional probabilities of unobserved variables with sigmoid units and Gaussian Mixtures respectively. Further improvements were presented in~\cite{uria2014deep,germain2015made}, that extend previous works by introducing a training strategy that copes with all possible autoregressive orderings among variables. Powerful generative models such as Pixel-RNN~\cite{oord2016pixel}, Pixel-CNN~\cite{van2016conditional} condition the probability distribution of pixels on previous ones, following a preset ordering. Recently, autoregression techniques have been merged with attention and meta-learning techniques for few-shot density estimation~\cite{reed2017few}, as well as the parallel framework of normalizing flows~\cite{rezende2015variational} in ~\cite{papamakarios2017masked}.


==> sections/related_bkp.tex <==
\section{Related work}
\label{sec:related}
\dvd{più guidati e strutturati}
{\bf Novelty and anomaly detection in vision.}
\dvd{still need to add \cite{hinami2017joint}}
\dvd{Add dataset by shah}
Novelty (anomaly) detection refers to the individuation, at test time, of examples drawn from a distribution different from the training one. This general formulation prevents the definition and labeling of novel examples; therefore, traditional approaches are dominated by unsupervised models, among which two main strategies emerge.
On the one hand, many works learn a parametric compression and reconstruction of normal data, assuming outliers will lead to higher residuals. Sparse-coding algorithms~\cite{zhao2011online,cong2011sparse,lu2013abnormal} adhere to such framework, and represent normal patterns as a linear combination of a set of basis components, imposing a sparsity constraint on scalar coefficients.
A complementary line of research focuses on probability distributions, employing different models to approximate the density function of normal appearance and motion features. In this respect, prior works involve both non-parametric~\cite{adam2008robust} and parametric~\cite{basharat2008learning,mahadevan2010anomaly,li2014anomaly} estimators, as well as graphical modeling~\cite{duong2005activity,kim2009observe,kwon2015unified}.
Finally, other unsupervised approaches involve crowd trajectory analysis~\cite{mehran2009abnormal, calderara2011detecting}, video volumes clustering~\cite{zhong2004detecting,roshtkhari2013online}, foreground explainability~\cite{antic2011video} and discriminability of normal frames with respect to context~\cite{del2016discriminative,ionescu2017unmasking}. For a comprehensive review of traditional anomaly detection techniques in computer vision, we refer the reader to~\cite{popoola2012video}.\\
As in most fields, the deep learning breakthrough affected novelty detection research in the choice of the features set: indeed, modern approaches employ deep representations in the expense of hand crafted features.
Standard algorithms such as one-class support vector machines (OC-SVM)~\cite{scholkopf2000support} or Gaussian classifiers are now employed out of latent representations extracted by deep networks~\cite{xu2017detecting,SABOKROU2018}.
Similairly, modern probabilistic models aim at estimating densities in deep feature space by means of Gaussian Mixtures~\cite{zong2018deep} or minimizing energy functions~\cite{zhai2016deep}.\dvd{Dire che (tipically) queste stime avvengono a posteriori, dopo il training. se è così.}
Nevertheless, reconstruction-based metrics still represent the most common choice, including autoencoders~\cite{hasan2016learning}, sparse coding with temporal constraints~\cite{luo2017revisit}, future frame prediction~\cite{liu2017future} and adversarially learned denoising networks~\cite{sabokrou2018adversarially}.
Motivated by their effectiveness in learning complex distributions, a very recent trend in literature involves training generative adversarial networks (GANs) on normal samples. Despite being powerful, such models approximate an implicit density function, meaning that they can be sampled from but not queried for likelihood values. Therefore, GAN-based novelty detection employ different heuristics for the evaluation. Specifically,~\cite{ravanbakhsh2017abnormal} employ reconstruction measures to monitor abnormalities, whereas~\cite{ravanbakhsh2017training} directly queries the discriminator for a normalcy score.\\
Finally, it is worth mentioning two research problems closely related to novelty detection. \emph{Outlier detection} refers to the identification of noisy samples \emph{within} a dataset, without a previous separate training on inliers only~\cite{xia2015learning,you2017provable}. Differently, \emph{out-of-distribution detection} identifies a regime in which a task supervision - such as a classification objective - is employed within the normal sample set, and novel samples are detected by means of the model's confidence~\cite{liang2017enhancing,hendrycks2016baseline,lee2017training}.\\\\
%
{\bf Autoregressive density estimation}
The first deep autoregressive models were introduced to overcome the issues affecting Restricted Boltzmann
Machines~\cite{smolensky1986information,freund1992fast} in modeling the density of binary inputs. NADE~\cite{larochelle2011neural} and its real-valued version RNADE~\cite{uria2013rnade} employ a deep network to estimate conditional probabilities of unobserved variables with sigmoid units and Gaussian Mixtures respectively. Further improvements were presented in~\cite{uria2014deep,germain2015made}, that extend previous works by introducing a training strategy copying with all possible autoregressive orderings among variables. When employed directly on color space, autoregression techniques lead to powerful generative models such as Pixel-RNN~\cite{oord2016pixel} and Pixel-CNN~\cite{van2016conditional}, capable of hallucinating new images sequentially and conditioning the probability distribution from which a pixel is sampled on previously sampled ones, following a preset ordering. Recently, autoregression techniques have been merged with attention and meta-learning techniques for few-shot density estimation~\cite{reed2017few}, as well as the parallel framework of normalizing flows in ~\cite{kingma2016improved,papamakarios2017masked}.

